Prediction of Handball Matches with Statistically Enhanced Learning via Estimated Team Strengths

We propose a Statistically Enhanced Learning (aka. SEL) model to predict handball games. Our Machine Learning model augmented with SEL features outperforms state-of-the-art models with an accuracy beyond 80%. In this work, we show how we construct the data set to train Machine Learning models on past female club matches. We then compare different models and evaluate them to assess their performance capabilities. Finally, explainability methods allow us to change the scope of our tool from a purely predictive solution to a highly insightful analytical tool. This can become a valuable asset for handball teams' coaches providing valuable statistical and predictive insights to prepare future competitions.

==> figures/tex/simulationCMP.tex <==
\begin{tikzpicture}
    \begin{axis}[xlabel=$\lambda$,
        ylabel=$\nu$,
        zlabel=Empirical mean,
        x dir=reverse,
        x tick label style={draw=none},
        y tick label style={draw=none},
        z tick label style={draw=none}]
    \addplot3 [surf, mesh/rows=10, only marks, scatter]
    table[x=lambda, y=nu, z=emp_mean, col sep=comma] {figures/data/CMP_simu.csv};
    \end{axis}
\end{tikzpicture}
